XDLM: Cross-lingual Diffusion Language Model for Machine Translation

Recently, diffusion models have excelled in image generation tasks and have also been applied to neural language processing (NLP) for controllable text generation. However, the application of diffusion models in a cross-lingual setting is less unexplored. Additionally, while pretraining with diffusion models has been studied within a single language, the potential of cross-lingual pretraining remains understudied. To address these gaps, we propose XDLM, a novel Cross-lingual diffusion model for machine translation, consisting of pretraining and fine-tuning stages. In the pretraining stage, we propose TLDM, a new training objective for mastering the mapping between different languages; in the fine-tuning stage, we build up the translation system based on the pretrained model. We evaluate the result on several machine translation benchmarks and outperformed both diffusion and Transformer baselines.

==> case_study.tex <==
\section{Case Study}
\label{sec:case_study}
In this section, we carry out a qualitative analysis to highlight the merits of our model by demonstrating the generated samples using the WMT14 dataset. Several representative samples are presented in Table 3.





Through comparison, we observe that the conventional RDM model struggles to grasp the mapping relationship between different language domains and is inclined to generate text with a blend of domains. Conversely, under the guidance of language embedding, our XDLM model proficiently masters the mapping relations between different languages. The sample also illustrates the enhanced speed of convergence exhibited by XDLM under the pretraining provided by TDLM.

%\begin{table}[]
%\centering
%\begin{tabular}{|c|l|l|}
%\hline
%\multicolumn{3}{|c|}{Source: Yesterday, Gutacht's Mayor gave a clear answer to this question.} \\
%\multicolumn{3}{|c|}{Target: Diese Frage hat Gutachs Bürgermeister gestern klar beantwortet.}  \\
%\hline
%Name & Iteration & Decodes \\
%\hline
%\multirow{RDM-Multinomial} & 0 & Content 1 \\
% & 1 & Content 2 \\
% & 2 & Content 3 \\
% & 3 & Content 4 \\
% & 4 & Content 5 \\
%\hline
%\multirow{XDLM} & 0 & Content 6 \\
% & 1 & Content 7 \\
% & 2 & Content 8 \\
% & 3 & Content 9 \\
% & 4 & Content 10 \\
%\hline
%\end{tabular}
%\caption{Qualitative samples of test paraphrases generated from different diffusion models. Words are in lower case}
%\label{table:your_label}
%\end{table}


